Competition-Level Code Generation with AlphaCode

Programming is a powerful and ubiquitous problem-solving tool. Developing systems that can assist programmers or even generate programs independently could make programming more productive and accessible, yet so far incorporating innovations in AI has proven challenging. Recent large-scale language models have demonstrated an impressive ability to generate code, and are now able to complete simple programming tasks. However, these models still perform poorly when evaluated on more complex, unseen problems that require problem-solving skills beyond simply translating instructions into code. For example, competitive programming problems which require an understanding of algorithms and complex natural language remain extremely challenging. To address this gap, we introduce AlphaCode, a system for code generation that can create novel solutions to these problems that require deeper reasoning. In simulated evaluations on recent programming competitions on the Codeforces platform, AlphaCode achieved on average a ranking of top 54.3% in competitions with more than 5,000 participants. We found that three key components were critical to achieve good and reliable performance: (1) an extensive and clean competitive programming dataset for training and evaluation, (2) large and efficient-to-sample transformer-based architectures, and (3) large-scale model sampling to explore the search space, followed by filtering based on program behavior to a small set of submissions.

==> figures/lcs_py_fastio_example.tex <==
\begin{figure}[h]
\begin{center}

\definecolor{lightorange}{RGB}{255,225,184}


\begin{lstlisting}[frame=tb] 
BUFSIZE = 8192

class FastIO(IOBase):
    newlines = 0

    def __init__(self, file):
        self._fd = file.fileno()
        self.buffer = BytesIO()
        self.writable = "x" in file.mode or "r" not in file.mode
        self.write = self.buffer.write if self.writable else None

    def read(self):
        while True:
            b = os.read(self._fd, max(os.fstat(self._fd).st_size, BUFSIZE))
            if not b:
                break
            ptr = self.buffer.tell()
            self.buffer.seek(0, 2), self.buffer.write(b), self.buffer.seek(ptr)
        self.newlines = 0
        return self.buffer.read()

    def readline(self):
        while self.newlines == 0:
            b = os.read(self._fd, max(os.fstat(self._fd).st_size, BUFSIZE))
            self.newlines = b.count(b"\n") + (not b)
            ptr = self.buffer.tell()
            self.buffer.seek(0, 2), self.buffer.write(b), self.buffer.seek(ptr)
        self.newlines -= 1
        return self.buffer.readline()

    def flush(self):
        if self.writable:
            os.write(self._fd, self.buffer.getvalue())
            self.buffer.truncate(0), self.buffer.seek(0)
\end{lstlisting}

\vspace{-0.3cm}
\caption{\textbf{LCS example}. An LCS of length 805 that appears 127 times (1.66\% of all human python validation solutions). In the appendix we provide further examples of very long LCS found in human solutions.
}
\label{fig:lcs_py_fastio}
\end{center}
\end{figure}

==> figures/limitations-subproblems.tex <==
\begin{figure}[t]
\begin{center}
\begin{minipage}[t]{.45\textwidth}
Solution to sqr\_conv problem:
\begin{lstlisting}[language=Python,basicstyle=\tiny\selectfont\ttfamily]
def replace(a):
    l = len(a)
    b = []
    for i in range(l):
        b.append(a[i]**2)
    return b

def add(a):
    l = len(a)
    b = []
    for i in range(l):
        if i == 0:
            b.append(a[i]+a[i+1])
        elif i == l-1:
            b.append(a[i]+a[i-1])
        else:
            b.append(a[i]+a[i-1]+a[i+1])
    return b

n = int(input())
a = list(map(int,input().split()))

ans = replace(a)
ans = add(ans)

for i in range(n):
    print(ans[i],end=' ')
print()
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{.45\textwidth}
Solution to inc\_\dots 9 times \dots \_inc problem:
\begin{lstlisting}[language=Python,basicstyle=\tiny\selectfont\ttfamily]
import sys

def read_input():
    input()
    a = list(map(int, input().split()))
    return a

def increment_arr(a):
    a = list(map(lambda x: x + 1, a))
    return a

def print_result(a):
    print(" ".join(map(str, a)))

def main():
    a = read_input()

    a = increment_arr(a)
    a = increment_arr(a)
    a = increment_arr(a)
    a = increment_arr(a)
    a = increment_arr(a)
    a = increment_arr(a)
    a = increment_arr(a)
    a = increment_arr(a)
    a = increment_arr(a)

    print_result(a)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{.45\textwidth}
Solution to inc\_mul2\_inc\_mul2\_inc\_mul2 problem:
\begin{lstlisting}[language=C++,basicstyle=\tiny\selectfont\ttfamily]
#include <bits/stdc++.h>
using namespace std;
void inc(vector<int> &v) {
  int n = v.size();
  for (int i = 0; i < n; i++) {
    v[i]++;
  }
}
void mult(vector<int> &v) {
  int n = v.size();
  for (int i = 0; i < n; i++) {
    v[i] *= 2;
  }
}
int main() {
  int n;
  cin >> n;
  vector<int> v(n);
  for (int i = 0; i < n; i++) {
    cin >> v[i];
  }
  inc(v);
  mult(v);
  inc(v);
  mult(v);
  inc(v);
  mult(v);
  for (int i = 0; i < n; i++) {
    cout << v[i] << " ";
  }
}
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{.45\textwidth}
Solution to inc\_inc\_mul2\_sqr \\ problem:
\begin{lstlisting}[language=Python,basicstyle=\tiny\selectfont\ttfamily]
def inc(a):
    for i in range(len(a)):
        a[i]+=1
    return a
def inc2(a):
    for i in range(len(a)):
        a[i]+=1
    return a
def mult(a):
    for i in range(len(a)):
        a[i]*=2
    return a
def sqr(a):
    for i in range(len(a)):
        a[i]=a[i]**2
    return a
n=int(input())
a=[int(i) for i in input().split()]
b=[]
for i in range(n):
    b.append(0)
for i in range(n):
    b[i]=a[i]
inc(b)
inc2(b)
mult(b)
sqr(b)
for i in range(n):
    print(b[i],end=' ')

\end{lstlisting}
\end{minipage}
\vspace{-0.4cm}
\caption{\textbf{Solutions to parameterized assignments where the model extracts a function for every requested command}. Note that in solution to inc\_inc\_mul2\_sqr problem the first and the second increment commands don't share the same function. In other solutions only unique functions are created and reused accordingly.}
\label{fig:subproblems-code}
\end{center}
\end{figure}

==> tables/limitations-no-consecutive-zeros-samples.tex <==


\begin{figure}[t]
\begin{center}
\begin{minipage}[t]{.55\textwidth}
Solution to the original problem:
\begin{lstlisting}[language=C++,basicstyle=\tiny\selectfont\ttfamily]
#include <bits/stdc++.h>
using namespace std;
const long long inf = 1e9 + 7;
long long read() {
  long long x = 0, f = 1;
  char ch = getchar();
  while (!isdigit(ch)) {
    if (ch == '-') f = -1;
    ch = getchar();
  }
  while (isdigit(ch)) x = x * 10 + ch - '0', ch = getchar();
  return f * x;
}
int n, m;
int a[400005], f[400005][3];
int main() {
  int t = read();
  while (t--) {
    n = read();
    memset(f, 0, sizeof(f));
    f[1][0] = 1, f[1][1] = 1;
    for (int i = 2; i <= n; i++) {
      f[i][0] = f[i - 1][0] + f[i - 1][1];
      f[i][1] = f[i - 1][0];
    }
    printf("%
  }
  return 0;
}
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{.35\textwidth}
Solution to the simplified problem:
\begin{lstlisting}[language=C++,basicstyle=\tiny\selectfont\ttfamily]
#include <bits/stdc++.h>
using namespace std;
int main() {
  int t;
  cin >> t;
  while (t--) {
    int n;
    cin >> n;
    long long ans = 0;
    long long a = 1;
    long long b = 1;
    for (int i = 1; i <= n; i++) {
      ans = a + b;
      a = b;
      b = ans;
    }
    cout << ans << endl;
  }
}
\end{lstlisting}
\end{minipage}
\vspace{-0.4cm}
\caption{\textbf{Solutions to the original and simplified versions of \emph{No Consecutive Zeros}}. Note that the original problem is solved with dynamic programming, with no reference to Fibonacci numbers.}
\label{fig:no-consecutive-zeros-code}
\end{center}
\end{figure}

==> tables/limitations-subproblems.tex <==
\begin{table}
\centering
\begin{tabular}{lr}
\toprule
Problem & Solve Rate \\   
\midrule
inc            & 17.948\% \\
inc\_inc       & 2.982\% \\
inc\_inc\_inc  & 0.236\% \\
inc\_\dots 6 times \dots \_inc & 0.009\% \\
inc\_\dots 9 times \dots \_inc & 0.007\% \\

mul2           & 19.051\% \\
mul2\_mul2     & 0.258\% \\
mul2\_\dots 6 times \dots \_mul2  & 0.047\% \\

sqr                 & 22.028\% \\
sqr\_sqr            & 1.636\% \\
sqr\_sqr\_sqr       & 0.219\% \\
sqr\_\dots 5 times \dots \_sqr  & 0.001\% \\

inc\_mul2       & 0.229\% \\
mul2\_inc       & 0.258\% \\
inc\_sqr        & 5.084\% \\
sqr\_inc        & 3.001\% \\
sqr\_mul2       & 2.529\% \\
mul2\_sqr       & 2.245\% \\

inc\_mul2\_inc        & 0.255\%  \\
inc\_mul2\_inc\_mul2  & 0.060\%  \\
inc\_mul2\_inc\_mul2\_inc\_mul2  & 0.017\%  \\
inc\_inc\_mul2\_sqr  & 0.037\% \\
inc\_inc\_sqr\_inc\_inc  & 0.001\% \\

conv       & 0.268\% \\
conv\_conv       & 0.003\% \\
conv\_inc        & 0.006\% \\
conv\_sqr        & 0.001\% \\
conv\_mul2        & 0.014\% \\
inc\_conv        & <0.001\% \\
mul2\_conv        & 0.008\% \\
sqr\_conv        & 0.055\% \\

\bottomrule
\end{tabular}
\caption{\textbf{Solve rates to parameterized assignments}. This evaluation was conducted using the 9B version of the model, sampling up to 1M solutions.}
\label{tab:seq_calc}
\end{table}

